a posteriori stabilized sixth-order finite volume scheme with adaptive stencil construction -- Basics for the 1D steady-state hyperbolic equations

We propose an adaptive stencil construction for high order accurate finite volume schemes aposteriori stabilized devoted to solve one-dimensional steady-state hyperbolic equations. High-accuracy (up to the sixth-order presently) is achieved thanks to polynomial reconstructions while stability is provided with an aposteriori MOOD method which controls the cell polynomial degree for eliminating non-physical oscillations in the vicinity of discontinuities. We supplemented this scheme with a stencil construction allowing to reduce even further the numerical dissipation. The stencil is shifted away from troubles (shocks, discontinuities, etc.) leading to less oscillating polynomial reconstructions. Experimented on linear, B\"urgers', and Euler equations, we demonstrate that the adaptive stencil technique manages to retrieve smooth solutions with optimal order of accuracy but also irregular ones without spurious oscillations. Moreover we numerically show that the approach allows to reduce the dissipation still maintaining the essentially non-oscillatory behavior.

==> exB/I=40/out_NLSfsolveV3_7MOODNew5210_Var0-P0/TableConvs.tex <==
\begin{frame}
\frametitle{Burgers | ex3 | convergence tables}
\captionsetup{labelformat=empty}
\tiny\setlength{\tabcolsep}{1pt}
\begin{table}[h]\centering
\caption{ex3 | MOODNew5210 | Var0-P0}
\begin{tabular}{@{}ccccccccccccccccccccc@{}}\toprule
$I$ & \multicolumn{4}{l}{$P=0,1,2,5$} & & \multicolumn{4}{l}{$P=1,2,5$} & & \multicolumn{4}{l}{$P=2,5$} & & \multicolumn{4}{l}{$P=5$} & 5-CPD \\\cline{2-5}\cline{7-10}\cline{12-15}\cline{17-20}
& $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & 
\\\midrule
40 & 1.4E$-$02 & --- & 7.5E$-$02 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & 240 \\
\bottomrule
\end{tabular}
\end{table}

\end{frame}


==> exB/I=40/out_NLSfsolveV3_7MOODNew5210_Var0-P0/TablePlots.tex <==
\begin{frame}
\frametitle{Burgers | ex3 | MOODNew5210 | Var0-P0}
\begin{tabular}{c}
$I=40$\\
\\
\includegraphics[width=0.25\textwidth]{../../examplesB/ex3/out_NLSfsolveV3_7MOODNew5210_Var0-P0/res-I40-3MOOD-Phi}\\
\includegraphics[width=0.25\textwidth]{../../examplesB/ex3/out_NLSfsolveV3_7MOODNew5210_Var0-P0/res-I40-3MOOD-PhiError}\\
\includegraphics[width=0.25\textwidth]{../../examplesB/ex3/out_NLSfsolveV3_7MOODNew5210_Var0-P0/res-I40-3MOOD-Res}\\
\end{tabular}
\end{frame}


==> exB/I=40/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/Detail-I40.tex <==
\begin{frame}
\frametitle{Burgers | ex3 | MOODNew5210 | Var0-P0 | $I=40$}
\begin{tabular}{ccc}
\includegraphics[width=0.33333\textwidth]{../../examplesB/ex3/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I40-1MOOD-Phi} & 
\includegraphics[width=0.33333\textwidth]{../../examplesB/ex3/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I40-2MOOD-Phi} & 
\includegraphics[width=0.33333\textwidth]{../../examplesB/ex3/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I40-3MOOD-Phi} \\
\includegraphics[width=0.33333\textwidth]{../../examplesB/ex3/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I40-1MOOD-PhiError} & 
\includegraphics[width=0.33333\textwidth]{../../examplesB/ex3/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I40-2MOOD-PhiError} & 
\includegraphics[width=0.33333\textwidth]{../../examplesB/ex3/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I40-3MOOD-PhiError} \\
\includegraphics[width=0.33333\textwidth]{../../examplesB/ex3/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I40-1MOOD-Res} & 
\includegraphics[width=0.33333\textwidth]{../../examplesB/ex3/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I40-2MOOD-Res} & 
\includegraphics[width=0.33333\textwidth]{../../examplesB/ex3/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I40-3MOOD-Res} \\
\end{tabular}
\end{frame}


==> exB/I=40/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/TableConvs.tex <==
\begin{frame}
\frametitle{Burgers | ex3 | convergence tables}
\captionsetup{labelformat=empty}
\tiny\setlength{\tabcolsep}{1pt}
\begin{table}[h]\centering
\caption{ex3 | DSv1New5210 | Var0-MOOD}
\begin{tabular}{@{}ccccccccccccccccccccc@{}}\toprule
$I$ & \multicolumn{4}{l}{$P=0,1,2,5$} & & \multicolumn{4}{l}{$P=1,2,5$} & & \multicolumn{4}{l}{$P=2,5$} & & \multicolumn{4}{l}{$P=5$} & 5-CPD \\\cline{2-5}\cline{7-10}\cline{12-15}\cline{17-20}
& $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & 
\\\midrule
40 & 2.5E$-$02 & --- & 1.6E$-$01 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & 240 \\
\bottomrule
\end{tabular}
\end{table}

\end{frame}


==> exB/I=40/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/TablePlots.tex <==
\begin{frame}
\frametitle{Burgers | ex3 | DSv1New5210 | Var0-MOOD}
\begin{tabular}{c}
$I=40$\\
\\
\includegraphics[width=0.25\textwidth]{../../examplesB/ex3/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/res-I40-4DS-Phi}\\
\includegraphics[width=0.25\textwidth]{../../examplesB/ex3/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/res-I40-4DS-PhiError}\\
\includegraphics[width=0.25\textwidth]{../../examplesB/ex3/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/res-I40-4DS-Res}\\
\end{tabular}
\end{frame}


==> exB/I=40/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/Detail-I40.tex <==
\begin{frame}
\frametitle{Burgers | ex3 | DSv1New5210 | Var0-MOOD | $I=40$}
\begin{tabular}{c}
\includegraphics[width=1\textwidth]{../../examplesB/ex3/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I40-4DS-Phi} \\
\includegraphics[width=1\textwidth]{../../examplesB/ex3/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I40-4DS-PhiError} \\
\includegraphics[width=1\textwidth]{../../examplesB/ex3/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I40-4DS-Res} \\
\end{tabular}
\end{frame}


==> exB/I=40/out_TMeuler_7MOODCla5210_Var0-P0Fixing/TableConvs.tex <==
\begin{frame}
\frametitle{Burgers | ex3 | convergence tables}
\captionsetup{labelformat=empty}
\tiny\setlength{\tabcolsep}{1pt}
\begin{table}[h]\centering
\caption{ex3 | MOODCla5210 | Var0-P0Fixing}
\begin{tabular}{@{}ccccccccccccccccccccc@{}}\toprule
$I$ & \multicolumn{4}{l}{$P=0,1,2,5$} & & \multicolumn{4}{l}{$P=1,2,5$} & & \multicolumn{4}{l}{$P=2,5$} & & \multicolumn{4}{l}{$P=5$} & 5-CPD \\\cline{2-5}\cline{7-10}\cline{12-15}\cline{17-20}
& $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & 
\\\midrule
40 & 1.3E$-$02 & --- & 8.0E$-$02 & --- & & 1.3E$-$02 & --- & 8.0E$-$02 & --- & & 1.7E$-$03 & --- & 2.0E$-$02 & --- & & 1.7E$-$03 & --- & 2.0E$-$02 & --- & 12 \\
\bottomrule
\end{tabular}
\end{table}

\end{frame}


==> exB/I=40/out_TMeuler_7MOODCla5210_Var0-P0Fixing/TablePlots.tex <==
\begin{frame}
\frametitle{Burgers | ex3 | MOODCla5210 | Var0-P0Fixing}
\begin{tabular}{c}
$I=40$\\
\\
\includegraphics[width=0.25\textwidth]{../../examplesB/ex3/out_TMeuler_7MOODCla5210_Var0-P0Fixing/res-I40-Phi}\\
\includegraphics[width=0.25\textwidth]{../../examplesB/ex3/out_TMeuler_7MOODCla5210_Var0-P0Fixing/res-I40-PhiError}\\
\includegraphics[width=0.25\textwidth]{../../examplesB/ex3/out_TMeuler_7MOODCla5210_Var0-P0Fixing/res-I40-Res}\\
\end{tabular}
\end{frame}


==> exB/I=40/out_TMeuler_7MOODNew5210_Var0-P0/TableConvs.tex <==
\begin{frame}
\frametitle{Burgers | ex3 | convergence tables}
\captionsetup{labelformat=empty}
\tiny\setlength{\tabcolsep}{1pt}
\begin{table}[h]\centering
\caption{ex3 | MOODNew5210 | Var0-P0}
\begin{tabular}{@{}ccccccccccccccccccccc@{}}\toprule
$I$ & \multicolumn{4}{l}{$P=0,1,2,5$} & & \multicolumn{4}{l}{$P=1,2,5$} & & \multicolumn{4}{l}{$P=2,5$} & & \multicolumn{4}{l}{$P=5$} & 5-CPD \\\cline{2-5}\cline{7-10}\cline{12-15}\cline{17-20}
& $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & 
\\\midrule
40 & 1.5E$-$02 & --- & 1.3E$-$01 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & 240 \\
\bottomrule
\end{tabular}
\end{table}

\end{frame}


==> exB/I=40/out_TMeuler_7MOODNew5210_Var0-P0/TablePlots.tex <==
\begin{frame}
\frametitle{Burgers | ex3 | MOODNew5210 | Var0-P0}
\begin{tabular}{c}
$I=40$\\
\\
\includegraphics[width=0.25\textwidth]{../../examplesB/ex3/out_TMeuler_7MOODNew5210_Var0-P0/res-I40-3MOOD-Phi}\\
\includegraphics[width=0.25\textwidth]{../../examplesB/ex3/out_TMeuler_7MOODNew5210_Var0-P0/res-I40-3MOOD-PhiError}\\
\includegraphics[width=0.25\textwidth]{../../examplesB/ex3/out_TMeuler_7MOODNew5210_Var0-P0/res-I40-3MOOD-Res}\\
\end{tabular}
\end{frame}


==> exB/I=40/out_TMeuler_7MOODNew5210_Var0-P0/iMOOD/Detail-I40.tex <==
\begin{frame}
\frametitle{Burgers | ex3 | MOODNew5210 | Var0-P0 | $I=40$}
\begin{tabular}{ccc}
\includegraphics[width=0.33333\textwidth]{../../examplesB/ex3/out_TMeuler_7MOODNew5210_Var0-P0/iMOOD/res-I40-1MOOD-Phi} & 
\includegraphics[width=0.33333\textwidth]{../../examplesB/ex3/out_TMeuler_7MOODNew5210_Var0-P0/iMOOD/res-I40-2MOOD-Phi} & 
\includegraphics[width=0.33333\textwidth]{../../examplesB/ex3/out_TMeuler_7MOODNew5210_Var0-P0/iMOOD/res-I40-3MOOD-Phi} \\
\includegraphics[width=0.33333\textwidth]{../../examplesB/ex3/out_TMeuler_7MOODNew5210_Var0-P0/iMOOD/res-I40-1MOOD-PhiError} & 
\includegraphics[width=0.33333\textwidth]{../../examplesB/ex3/out_TMeuler_7MOODNew5210_Var0-P0/iMOOD/res-I40-2MOOD-PhiError} & 
\includegraphics[width=0.33333\textwidth]{../../examplesB/ex3/out_TMeuler_7MOODNew5210_Var0-P0/iMOOD/res-I40-3MOOD-PhiError} \\
\includegraphics[width=0.33333\textwidth]{../../examplesB/ex3/out_TMeuler_7MOODNew5210_Var0-P0/iMOOD/res-I40-1MOOD-Res} & 
\includegraphics[width=0.33333\textwidth]{../../examplesB/ex3/out_TMeuler_7MOODNew5210_Var0-P0/iMOOD/res-I40-2MOOD-Res} & 
\includegraphics[width=0.33333\textwidth]{../../examplesB/ex3/out_TMeuler_7MOODNew5210_Var0-P0/iMOOD/res-I40-3MOOD-Res} \\
\end{tabular}
\end{frame}


==> exB/I=40/out_TMeuler_8DSv1Cla5210_Var0-MOODFixing/TableConvs.tex <==
\begin{frame}
\frametitle{Burgers | ex3 | convergence tables}
\captionsetup{labelformat=empty}
\tiny\setlength{\tabcolsep}{1pt}
\begin{table}[h]\centering
\caption{ex3 | DSv1Cla5210 | Var0-MOODFixing}
\begin{tabular}{@{}ccccccccccccccccccccc@{}}\toprule
$I$ & \multicolumn{4}{l}{$P=0,1,2,5$} & & \multicolumn{4}{l}{$P=1,2,5$} & & \multicolumn{4}{l}{$P=2,5$} & & \multicolumn{4}{l}{$P=5$} & 5-CPD \\\cline{2-5}\cline{7-10}\cline{12-15}\cline{17-20}
& $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & 
\\\midrule
40 & 2.6E$-$02 & --- & 1.8E$-$01 & --- & & 2.6E$-$02 & --- & 1.8E$-$01 & --- & & 2.6E$-$02 & --- & 1.8E$-$01 & --- & & 2.6E$-$02 & --- & 1.8E$-$01 & --- & 0 \\
\bottomrule
\end{tabular}
\end{table}

\end{frame}


==> exB/I=40/out_TMeuler_8DSv1Cla5210_Var0-MOODFixing/TablePlots.tex <==
\begin{frame}
\frametitle{Burgers | ex3 | DSv1Cla5210 | Var0-MOODFixing}
\begin{tabular}{c}
$I=40$\\
\\
\includegraphics[width=0.25\textwidth]{../../examplesB/ex3/out_TMeuler_8DSv1Cla5210_Var0-MOODFixing/res-I40-Phi}\\
\includegraphics[width=0.25\textwidth]{../../examplesB/ex3/out_TMeuler_8DSv1Cla5210_Var0-MOODFixing/res-I40-PhiError}\\
\includegraphics[width=0.25\textwidth]{../../examplesB/ex3/out_TMeuler_8DSv1Cla5210_Var0-MOODFixing/res-I40-Res}\\
\end{tabular}
\end{frame}


==> exB/I=40/out_TMeuler_8DSv1New5210_Var0-MOOD/TableConvs.tex <==
\begin{frame}
\frametitle{Burgers | ex3 | convergence tables}
\captionsetup{labelformat=empty}
\tiny\setlength{\tabcolsep}{1pt}
\begin{table}[h]\centering
\caption{ex3 | DSv1New5210 | Var0-MOOD}
\begin{tabular}{@{}ccccccccccccccccccccc@{}}\toprule
$I$ & \multicolumn{4}{l}{$P=0,1,2,5$} & & \multicolumn{4}{l}{$P=1,2,5$} & & \multicolumn{4}{l}{$P=2,5$} & & \multicolumn{4}{l}{$P=5$} & 5-CPD \\\cline{2-5}\cline{7-10}\cline{12-15}\cline{17-20}
& $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & 
\\\midrule
40 & 2.6E$-$02 & --- & 2.1E$-$01 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & 240 \\
\bottomrule
\end{tabular}
\end{table}

\end{frame}


==> exB/I=40/out_TMeuler_8DSv1New5210_Var0-MOOD/TablePlots.tex <==
\begin{frame}
\frametitle{Burgers | ex3 | DSv1New5210 | Var0-MOOD}
\begin{tabular}{c}
$I=40$\\
\\
\includegraphics[width=0.25\textwidth]{../../examplesB/ex3/out_TMeuler_8DSv1New5210_Var0-MOOD/res-I40-4DS-Phi}\\
\includegraphics[width=0.25\textwidth]{../../examplesB/ex3/out_TMeuler_8DSv1New5210_Var0-MOOD/res-I40-4DS-PhiError}\\
\includegraphics[width=0.25\textwidth]{../../examplesB/ex3/out_TMeuler_8DSv1New5210_Var0-MOOD/res-I40-4DS-Res}\\
\end{tabular}
\end{frame}


==> exB/I=40/out_TMeuler_8DSv1New5210_Var0-MOOD/iMOOD/Detail-I40.tex <==
\begin{frame}
\frametitle{Burgers | ex3 | DSv1New5210 | Var0-MOOD | $I=40$}
\begin{tabular}{c}
\includegraphics[width=1\textwidth]{../../examplesB/ex3/out_TMeuler_8DSv1New5210_Var0-MOOD/iMOOD/res-I40-4DS-Phi} \\
\includegraphics[width=1\textwidth]{../../examplesB/ex3/out_TMeuler_8DSv1New5210_Var0-MOOD/iMOOD/res-I40-4DS-PhiError} \\
\includegraphics[width=1\textwidth]{../../examplesB/ex3/out_TMeuler_8DSv1New5210_Var0-MOOD/iMOOD/res-I40-4DS-Res} \\
\end{tabular}
\end{frame}


==> exE/I=40_80/out_NLSfsolveV3_7MOODNew5210_Var0-P0/TableConvs.tex <==
\begin{frame}
\frametitle{Euler | ex1 | convergence tables}
\captionsetup{labelformat=empty}
\tiny\setlength{\tabcolsep}{1pt}
\begin{table}[h]\centering
\caption{ex1/SupSuba | MOODNew5210 | Var0-P0}
\begin{tabular}{@{}ccccccccccccccccccccc@{}}\toprule
$I$ & \multicolumn{4}{l}{$P=0,1,2,5$} & & \multicolumn{4}{l}{$P=1,2,5$} & & \multicolumn{4}{l}{$P=2,5$} & & \multicolumn{4}{l}{$P=5$} & 5-CPD \\\cline{2-5}\cline{7-10}\cline{12-15}\cline{17-20}
& $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & 
\\\midrule
40 & 4.2E$-$03 & --- & 7.9E$-$02 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & 0 \\
80 & 1.9E$-$03 & 1.1 & 7.6E$-$02 & 0.1 & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & 480 \\
\bottomrule
\end{tabular}
\end{table}

\end{frame}


==> exE/I=40_80/out_NLSfsolveV3_7MOODNew5210_Var0-P0/TablePlots.tex <==
\begin{frame}
\frametitle{Euler | ex1/SupSuba | MOODNew5210 | Var0-P0}
\begin{tabular}{cc}
$I=40$ & $I=80$\\
 & \\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/res-I40-4MOOD-Rho} &
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/res-I80-4MOOD-Rho}\\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/res-I40-4MOOD-RhoError} &
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/res-I80-4MOOD-RhoError}\\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/res-I40-4MOOD-Res} &
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/res-I80-4MOOD-Res}\\
\end{tabular}
\end{frame}


==> exE/I=40_80/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/Detail-I20.tex <==
\begin{frame}
\frametitle{Euler | ex1/SupSuba | MOODNew5210 | Var0-P0 | $I=20$}
\begin{tabular}{cccc}
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I20-1MOOD-Rho} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I20-2MOOD-Rho} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I20-3MOOD-Rho} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I20-4MOOD-Rho} \\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I20-1MOOD-RhoError} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I20-2MOOD-RhoError} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I20-3MOOD-RhoError} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I20-4MOOD-RhoError} \\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I20-1MOOD-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I20-2MOOD-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I20-3MOOD-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I20-4MOOD-Res} \\
\end{tabular}
\end{frame}


==> exE/I=40_80/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/Detail-I40.tex <==
\begin{frame}
\frametitle{Euler | ex1/SupSuba | MOODNew5210 | Var0-P0 | $I=40$}
\begin{tabular}{cccc}
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I40-1MOOD-Rho} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I40-2MOOD-Rho} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I40-3MOOD-Rho} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I40-4MOOD-Rho} \\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I40-1MOOD-RhoError} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I40-2MOOD-RhoError} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I40-3MOOD-RhoError} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I40-4MOOD-RhoError} \\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I40-1MOOD-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I40-2MOOD-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I40-3MOOD-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I40-4MOOD-Res} \\
\end{tabular}
\end{frame}


==> exE/I=40_80/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/Detail-I80.tex <==
\begin{frame}
\frametitle{Euler | ex1/SupSuba | MOODNew5210 | Var0-P0 | $I=80$}
\begin{tabular}{cccc}
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I80-1MOOD-Rho} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I80-2MOOD-Rho} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I80-3MOOD-Rho} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I80-4MOOD-Rho} \\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I80-1MOOD-RhoError} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I80-2MOOD-RhoError} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I80-3MOOD-RhoError} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I80-4MOOD-RhoError} \\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I80-1MOOD-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I80-2MOOD-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I80-3MOOD-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I80-4MOOD-Res} \\
\end{tabular}
\end{frame}


==> exE/I=40_80/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/TableConvs.tex <==
\begin{frame}
\frametitle{Euler | ex1 | convergence tables}
\captionsetup{labelformat=empty}
\tiny\setlength{\tabcolsep}{1pt}
\begin{table}[h]\centering
\caption{ex1/SupSuba | DSv1New5210 | Var0-MOOD}
\begin{tabular}{@{}ccccccccccccccccccccc@{}}\toprule
$I$ & \multicolumn{4}{l}{$P=0,1,2,5$} & & \multicolumn{4}{l}{$P=1,2,5$} & & \multicolumn{4}{l}{$P=2,5$} & & \multicolumn{4}{l}{$P=5$} & 5-CPD \\\cline{2-5}\cline{7-10}\cline{12-15}\cline{17-20}
& $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & 
\\\midrule
40 & 7.2E$-$03 & --- & 1.4E$-$01 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & 0 \\
80 & 3.6E$-$03 & 1.0 & 1.4E$-$01 & 0.0 & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & 480 \\
\bottomrule
\end{tabular}
\end{table}

\end{frame}


==> exE/I=40_80/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/TablePlots.tex <==
\begin{frame}
\frametitle{Euler | ex1/SupSuba | DSv1New5210 | Var0-MOOD}
\begin{tabular}{cc}
$I=40$ & $I=80$\\
 & \\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/res-I40-8DS-Rho} &
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/res-I80-8DS-Rho}\\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/res-I40-8DS-RhoError} &
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/res-I80-8DS-RhoError}\\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/res-I40-8DS-Res} &
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/res-I80-8DS-Res}\\
\end{tabular}
\end{frame}


==> exE/I=40_80/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/Detail-I20.tex <==
\begin{frame}
\frametitle{Euler | ex1/SupSuba | DSv1New5210 | Var0-MOOD | $I=20$}
\begin{tabular}{ccccc}
\includegraphics[width=0.2\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I20-5DS-Rho} & 
\includegraphics[width=0.2\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I20-6DS-Rho} & 
\includegraphics[width=0.2\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I20-7DS-Rho} & 
\includegraphics[width=0.2\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I20-8DS-Rho} & 
\includegraphics[width=0.2\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I20-9DS-Rho} \\
\includegraphics[width=0.2\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I20-5DS-RhoError} & 
\includegraphics[width=0.2\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I20-6DS-RhoError} & 
\includegraphics[width=0.2\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I20-7DS-RhoError} & 
\includegraphics[width=0.2\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I20-8DS-RhoError} & 
\includegraphics[width=0.2\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I20-9DS-RhoError} \\
\includegraphics[width=0.2\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I20-5DS-Res} & 
\includegraphics[width=0.2\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I20-6DS-Res} & 
\includegraphics[width=0.2\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I20-7DS-Res} & 
\includegraphics[width=0.2\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I20-8DS-Res} & 
\includegraphics[width=0.2\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I20-9DS-Res} \\
\end{tabular}
\end{frame}


==> exE/I=40_80/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/Detail-I40.tex <==
\begin{frame}
\frametitle{Euler | ex1/SupSuba | DSv1New5210 | Var0-MOOD | $I=40$}
\begin{tabular}{cccc}
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I40-5DS-Rho} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I40-6DS-Rho} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I40-7DS-Rho} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I40-8DS-Rho} \\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I40-5DS-RhoError} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I40-6DS-RhoError} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I40-7DS-RhoError} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I40-8DS-RhoError} \\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I40-5DS-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I40-6DS-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I40-7DS-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I40-8DS-Res} \\
\end{tabular}
\end{frame}


==> exE/I=40_80/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/Detail-I80.tex <==
\begin{frame}
\frametitle{Euler | ex1/SupSuba | DSv1New5210 | Var0-MOOD | $I=80$}
\begin{tabular}{cccc}
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I80-5DS-Rho} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I80-6DS-Rho} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I80-7DS-Rho} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I80-8DS-Rho} \\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I80-5DS-RhoError} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I80-6DS-RhoError} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I80-7DS-RhoError} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I80-8DS-RhoError} \\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I80-5DS-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I80-6DS-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I80-7DS-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSuba/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I80-8DS-Res} \\
\end{tabular}
\end{frame}


==> exE/I=41_81/out_NLSfsolveV3_7MOODNew5210_Var0-P0/TableConvs.tex <==
\begin{frame}
\frametitle{Euler | ex1 | convergence tables}
\captionsetup{labelformat=empty}
\tiny\setlength{\tabcolsep}{1pt}
\begin{table}[h]\centering
\caption{ex1/SupSubb | MOODNew5210 | Var0-P0}
\begin{tabular}{@{}ccccccccccccccccccccc@{}}\toprule
$I$ & \multicolumn{4}{l}{$P=0,1,2,5$} & & \multicolumn{4}{l}{$P=1,2,5$} & & \multicolumn{4}{l}{$P=2,5$} & & \multicolumn{4}{l}{$P=5$} & 5-CPD \\\cline{2-5}\cline{7-10}\cline{12-15}\cline{17-20}
& $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & 
\\\midrule
41 & 1.1E$-$02 & --- & 2.1E$-$01 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & 0 \\
81 & 5.3E$-$03 & 1.1 & 2.0E$-$01 & 0.0 & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & 486 \\
\bottomrule
\end{tabular}
\end{table}

\end{frame}


==> exE/I=41_81/out_NLSfsolveV3_7MOODNew5210_Var0-P0/TablePlots.tex <==
\begin{frame}
\frametitle{Euler | ex1/SupSubb | MOODNew5210 | Var0-P0}
\begin{tabular}{cc}
$I=41$ & $I=81$\\
 & \\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/res-I41-4MOOD-Rho} &
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/res-I81-4MOOD-Rho}\\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/res-I41-4MOOD-RhoError} &
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/res-I81-4MOOD-RhoError}\\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/res-I41-4MOOD-Res} &
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/res-I81-4MOOD-Res}\\
\end{tabular}
\end{frame}


==> exE/I=41_81/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/Detail-I21.tex <==
\begin{frame}
\frametitle{Euler | ex1/SupSubb | MOODNew5210 | Var0-P0 | $I=21$}
\begin{tabular}{cccc}
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I21-1MOOD-Rho} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I21-2MOOD-Rho} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I21-3MOOD-Rho} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I21-4MOOD-Rho} \\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I21-1MOOD-RhoError} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I21-2MOOD-RhoError} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I21-3MOOD-RhoError} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I21-4MOOD-RhoError} \\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I21-1MOOD-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I21-2MOOD-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I21-3MOOD-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I21-4MOOD-Res} \\
\end{tabular}
\end{frame}


==> exE/I=41_81/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/Detail-I41.tex <==
\begin{frame}
\frametitle{Euler | ex1/SupSubb | MOODNew5210 | Var0-P0 | $I=41$}
\begin{tabular}{cccc}
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I41-1MOOD-Rho} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I41-2MOOD-Rho} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I41-3MOOD-Rho} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I41-4MOOD-Rho} \\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I41-1MOOD-RhoError} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I41-2MOOD-RhoError} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I41-3MOOD-RhoError} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I41-4MOOD-RhoError} \\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I41-1MOOD-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I41-2MOOD-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I41-3MOOD-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I41-4MOOD-Res} \\
\end{tabular}
\end{frame}


==> exE/I=41_81/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/Detail-I81.tex <==
\begin{frame}
\frametitle{Euler | ex1/SupSubb | MOODNew5210 | Var0-P0 | $I=81$}
\begin{tabular}{cccc}
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I81-1MOOD-Rho} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I81-2MOOD-Rho} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I81-3MOOD-Rho} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I81-4MOOD-Rho} \\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I81-1MOOD-RhoError} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I81-2MOOD-RhoError} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I81-3MOOD-RhoError} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I81-4MOOD-RhoError} \\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I81-1MOOD-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I81-2MOOD-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I81-3MOOD-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_7MOODNew5210_Var0-P0/iMOOD/res-I81-4MOOD-Res} \\
\end{tabular}
\end{frame}


==> exE/I=41_81/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/TableConvs.tex <==
\begin{frame}
\frametitle{Euler | ex1 | convergence tables}
\captionsetup{labelformat=empty}
\tiny\setlength{\tabcolsep}{1pt}
\begin{table}[h]\centering
\caption{ex1/SupSubb | DSv1New5210 | Var0-MOOD}
\begin{tabular}{@{}ccccccccccccccccccccc@{}}\toprule
$I$ & \multicolumn{4}{l}{$P=0,1,2,5$} & & \multicolumn{4}{l}{$P=1,2,5$} & & \multicolumn{4}{l}{$P=2,5$} & & \multicolumn{4}{l}{$P=5$} & 5-CPD \\\cline{2-5}\cline{7-10}\cline{12-15}\cline{17-20}
& $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & 
\\\midrule
41 & 1.1E$-$02 & --- & 2.1E$-$01 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & 0 \\
81 & 5.2E$-$03 & 1.1 & 2.0E$-$01 & 0.0 & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & 486 \\
\bottomrule
\end{tabular}
\end{table}

\end{frame}


==> exE/I=41_81/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/TablePlots.tex <==
\begin{frame}
\frametitle{Euler | ex1/SupSubb | DSv1New5210 | Var0-MOOD}
\begin{tabular}{cc}
$I=41$ & $I=81$\\
 & \\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/res-I41-11DS-Rho} &
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/res-I81-11DS-Rho}\\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/res-I41-11DS-RhoError} &
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/res-I81-11DS-RhoError}\\
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/res-I41-11DS-Res} &
\includegraphics[width=0.25\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/res-I81-11DS-Res}\\
\end{tabular}
\end{frame}


==> exE/I=41_81/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/Detail-I21.tex <==
\begin{frame}
\frametitle{Euler | ex1/SupSubb | DSv1New5210 | Var0-MOOD | $I=21$}
\begin{tabular}{ccccccc}
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I21-5DS-Rho} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I21-6DS-Rho} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I21-7DS-Rho} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I21-8DS-Rho} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I21-9DS-Rho} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I21-10DS-Rho} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I21-11DS-Rho} \\
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I21-5DS-RhoError} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I21-6DS-RhoError} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I21-7DS-RhoError} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I21-8DS-RhoError} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I21-9DS-RhoError} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I21-10DS-RhoError} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I21-11DS-RhoError} \\
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I21-5DS-Res} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I21-6DS-Res} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I21-7DS-Res} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I21-8DS-Res} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I21-9DS-Res} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I21-10DS-Res} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I21-11DS-Res} \\
\end{tabular}
\end{frame}


==> exE/I=41_81/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/Detail-I41.tex <==
\begin{frame}
\frametitle{Euler | ex1/SupSubb | DSv1New5210 | Var0-MOOD | $I=41$}
\begin{tabular}{ccccccc}
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I41-5DS-Rho} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I41-6DS-Rho} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I41-7DS-Rho} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I41-8DS-Rho} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I41-9DS-Rho} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I41-10DS-Rho} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I41-11DS-Rho} \\
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I41-5DS-RhoError} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I41-6DS-RhoError} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I41-7DS-RhoError} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I41-8DS-RhoError} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I41-9DS-RhoError} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I41-10DS-RhoError} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I41-11DS-RhoError} \\
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I41-5DS-Res} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I41-6DS-Res} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I41-7DS-Res} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I41-8DS-Res} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I41-9DS-Res} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I41-10DS-Res} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I41-11DS-Res} \\
\end{tabular}
\end{frame}


==> exE/I=41_81/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/Detail-I81.tex <==
\begin{frame}
\frametitle{Euler | ex1/SupSubb | DSv1New5210 | Var0-MOOD | $I=81$}
\begin{tabular}{ccccccc}
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I81-5DS-Rho} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I81-6DS-Rho} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I81-7DS-Rho} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I81-8DS-Rho} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I81-9DS-Rho} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I81-10DS-Rho} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I81-11DS-Rho} \\
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I81-5DS-RhoError} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I81-6DS-RhoError} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I81-7DS-RhoError} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I81-8DS-RhoError} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I81-9DS-RhoError} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I81-10DS-RhoError} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I81-11DS-RhoError} \\
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I81-5DS-Res} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I81-6DS-Res} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I81-7DS-Res} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I81-8DS-Res} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I81-9DS-Res} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I81-10DS-Res} & 
\includegraphics[width=0.14286\textwidth]{../../examplesE/ex1/SupSubb/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD/iMOOD/res-I81-11DS-Res} \\
\end{tabular}
\end{frame}


==> exL/ex1_I=40/out_LSgauss_7MOODNew5210/TableConvs.tex <==
\begin{frame}
\frametitle{Linear | ex1 | convergence tables}
\captionsetup{labelformat=empty}
\tiny\setlength{\tabcolsep}{1pt}
\begin{table}[h]\centering
\caption{ex1 | MOODNew5210}
\begin{tabular}{@{}ccccccccccccccccccccc@{}}\toprule
$I$ & \multicolumn{4}{l}{$P=0,1,2,5$} & & \multicolumn{4}{l}{$P=1,2,5$} & & \multicolumn{4}{l}{$P=2,5$} & & \multicolumn{4}{l}{$P=5$} & 5-CPD \\\cline{2-5}\cline{7-10}\cline{12-15}\cline{17-20}
& $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & 
\\\midrule
40 & 1.1E$-$05 & --- & 6.9E$-$05 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & 0 \\
80 & 1.7E$-$07 & 6.0 & 1.4E$-$06 & 5.6 & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & 0 \\
160 & 2.6E$-$09 & 6.0 & 2.4E$-$08 & 5.9 & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & 960 \\
\bottomrule
\end{tabular}
\end{table}

\end{frame}


==> exL/ex1_I=40/out_LSgauss_7MOODNew5210/TablePlots.tex <==
\begin{frame}
\frametitle{Linear | ex1 | MOODNew5210}
\begin{tabular}{ccc}
$I=40$ & $I=80$ & $I=160$\\
 &  & \\
\includegraphics[width=0.25\textwidth]{../../examplesL/ex1/out_LSgauss_7MOODNew5210/res-I40-1MOOD-Phi} &
\includegraphics[width=0.25\textwidth]{../../examplesL/ex1/out_LSgauss_7MOODNew5210/res-I80-1MOOD-Phi} &
\includegraphics[width=0.25\textwidth]{../../examplesL/ex1/out_LSgauss_7MOODNew5210/res-I160-1MOOD-Phi}\\
\includegraphics[width=0.25\textwidth]{../../examplesL/ex1/out_LSgauss_7MOODNew5210/res-I40-1MOOD-PhiError} &
\includegraphics[width=0.25\textwidth]{../../examplesL/ex1/out_LSgauss_7MOODNew5210/res-I80-1MOOD-PhiError} &
\includegraphics[width=0.25\textwidth]{../../examplesL/ex1/out_LSgauss_7MOODNew5210/res-I160-1MOOD-PhiError}\\
\end{tabular}
\end{frame}


==> exL/ex1_I=40/out_LSgauss_7MOODNew5210/iMOOD/Detail-I160.tex <==
\begin{frame}
\frametitle{Linear | ex1 | MOODNew5210 | $I=160$}
\begin{tabular}{c}
\includegraphics[width=1\textwidth]{../../examplesL/ex1/out_LSgauss_7MOODNew5210/iMOOD/res-I160-1MOOD-Phi} \\
\includegraphics[width=1\textwidth]{../../examplesL/ex1/out_LSgauss_7MOODNew5210/iMOOD/res-I160-1MOOD-PhiError} \\
\end{tabular}
\end{frame}


==> exL/ex1_I=40/out_LSgauss_7MOODNew5210/iMOOD/Detail-I40.tex <==
\begin{frame}
\frametitle{Linear | ex1 | MOODNew5210 | $I=40$}
\begin{tabular}{c}
\includegraphics[width=1\textwidth]{../../examplesL/ex1/out_LSgauss_7MOODNew5210/iMOOD/res-I40-1MOOD-Phi} \\
\includegraphics[width=1\textwidth]{../../examplesL/ex1/out_LSgauss_7MOODNew5210/iMOOD/res-I40-1MOOD-PhiError} \\
\end{tabular}
\end{frame}


==> exL/ex1_I=40/out_LSgauss_7MOODNew5210/iMOOD/Detail-I80.tex <==
\begin{frame}
\frametitle{Linear | ex1 | MOODNew5210 | $I=80$}
\begin{tabular}{c}
\includegraphics[width=1\textwidth]{../../examplesL/ex1/out_LSgauss_7MOODNew5210/iMOOD/res-I80-1MOOD-Phi} \\
\includegraphics[width=1\textwidth]{../../examplesL/ex1/out_LSgauss_7MOODNew5210/iMOOD/res-I80-1MOOD-PhiError} \\
\end{tabular}
\end{frame}


==> exL/ex3_I=40/out_LSgauss_7MOODNew5210/TableConvs.tex <==
\begin{frame}
\frametitle{Linear | ex3 | convergence tables}
\captionsetup{labelformat=empty}
\tiny\setlength{\tabcolsep}{1pt}
\begin{table}[h]\centering
\caption{ex3 | MOODNew5210}
\begin{tabular}{@{}ccccccccccccccccccccc@{}}\toprule
$I$ & \multicolumn{4}{l}{$P=0,1,2,5$} & & \multicolumn{4}{l}{$P=1,2,5$} & & \multicolumn{4}{l}{$P=2,5$} & & \multicolumn{4}{l}{$P=5$} & 5-CPD \\\cline{2-5}\cline{7-10}\cline{12-15}\cline{17-20}
& $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & 
\\\midrule
40 & 4.4E$-$04 & --- & 8.4E$-$03 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & 240 \\
\bottomrule
\end{tabular}
\end{table}

\end{frame}


==> exL/ex3_I=40/out_LSgauss_7MOODNew5210/TablePlots.tex <==
\begin{frame}
\frametitle{Linear | ex3 | MOODNew5210}
\begin{tabular}{c}
$I=40$\\
\\
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_LSgauss_7MOODNew5210/res-I40-4MOOD-Phi}\\
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_LSgauss_7MOODNew5210/res-I40-4MOOD-PhiError}\\
\end{tabular}
\end{frame}


==> exL/ex3_I=40/out_LSgauss_7MOODNew5210/iMOOD/Detail-I40.tex <==
\begin{frame}
\frametitle{Linear | ex3 | MOODNew5210 | $I=40$}
\begin{tabular}{cccc}
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_LSgauss_7MOODNew5210/iMOOD/res-I40-1MOOD-Phi} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_LSgauss_7MOODNew5210/iMOOD/res-I40-2MOOD-Phi} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_LSgauss_7MOODNew5210/iMOOD/res-I40-3MOOD-Phi} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_LSgauss_7MOODNew5210/iMOOD/res-I40-4MOOD-Phi} \\
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_LSgauss_7MOODNew5210/iMOOD/res-I40-1MOOD-PhiError} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_LSgauss_7MOODNew5210/iMOOD/res-I40-2MOOD-PhiError} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_LSgauss_7MOODNew5210/iMOOD/res-I40-3MOOD-PhiError} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_LSgauss_7MOODNew5210/iMOOD/res-I40-4MOOD-PhiError} \\
\end{tabular}
\end{frame}


==> exL/ex3_I=40/out_LSgauss_8DSv1New5210/TableConvs.tex <==
\begin{frame}
\frametitle{Linear | ex3 | convergence tables}
\captionsetup{labelformat=empty}
\tiny\setlength{\tabcolsep}{1pt}
\begin{table}[h]\centering
\caption{ex3 | DSv1New5210}
\begin{tabular}{@{}ccccccccccccccccccccc@{}}\toprule
$I$ & \multicolumn{4}{l}{$P=0,1,2,5$} & & \multicolumn{4}{l}{$P=1,2,5$} & & \multicolumn{4}{l}{$P=2,5$} & & \multicolumn{4}{l}{$P=5$} & 5-CPD \\\cline{2-5}\cline{7-10}\cline{12-15}\cline{17-20}
& $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & 
\\\midrule
40 & 2.7E$-$04 & --- & 4.6E$-$03 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & 240 \\
\bottomrule
\end{tabular}
\end{table}

\end{frame}


==> exL/ex3_I=40/out_LSgauss_8DSv1New5210/TablePlots.tex <==
\begin{frame}
\frametitle{Linear | ex3 | DSv1New5210}
\begin{tabular}{c}
$I=40$\\
\\
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_LSgauss_8DSv1New5210/res-I40-8DS-Phi}\\
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_LSgauss_8DSv1New5210/res-I40-8DS-PhiError}\\
\end{tabular}
\end{frame}


==> exL/ex3_I=40/out_LSgauss_8DSv1New5210/iMOOD/Detail-I40.tex <==
\begin{frame}
\frametitle{Linear | ex3 | DSv1New5210 | $I=40$}
\begin{tabular}{cccc}
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_LSgauss_8DSv1New5210/iMOOD/res-I40-5DS-Phi} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_LSgauss_8DSv1New5210/iMOOD/res-I40-6DS-Phi} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_LSgauss_8DSv1New5210/iMOOD/res-I40-7DS-Phi} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_LSgauss_8DSv1New5210/iMOOD/res-I40-8DS-Phi} \\
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_LSgauss_8DSv1New5210/iMOOD/res-I40-5DS-PhiError} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_LSgauss_8DSv1New5210/iMOOD/res-I40-6DS-PhiError} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_LSgauss_8DSv1New5210/iMOOD/res-I40-7DS-PhiError} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_LSgauss_8DSv1New5210/iMOOD/res-I40-8DS-PhiError} \\
\end{tabular}
\end{frame}


==> exL/ex3_I=40/out_TMeuler_7MOODCla5210_Special10_Var0-P0Fixing/TableConvs.tex <==
\begin{frame}
\frametitle{Linear | ex3 | convergence tables}
\captionsetup{labelformat=empty}
\tiny\setlength{\tabcolsep}{1pt}
\begin{table}[h]\centering
\caption{ex3 | MOODCla5210Special10 | Var0-P0Fixing}
\begin{tabular}{@{}ccccccccccccccccccccc@{}}\toprule
$I$ & \multicolumn{4}{l}{$P=0,1,2,5$} & & \multicolumn{4}{l}{$P=1,2,5$} & & \multicolumn{4}{l}{$P=2,5$} & & \multicolumn{4}{l}{$P=5$} & 5-CPD \\\cline{2-5}\cline{7-10}\cline{12-15}\cline{17-20}
& $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & 
\\\midrule
40 & 4.5E$-$04 & --- & 8.4E$-$03 & --- & & 3.5E$-$04 & --- & 8.4E$-$03 & --- & & 3.5E$-$04 & --- & 8.4E$-$03 & --- & & 3.5E$-$04 & --- & 8.4E$-$03 & --- & 10 \\
\bottomrule
\end{tabular}
\end{table}

\end{frame}


==> exL/ex3_I=40/out_TMeuler_7MOODCla5210_Special10_Var0-P0Fixing/TablePlots.tex <==
\begin{frame}
\frametitle{Linear | ex3 | MOODCla5210Special10 | Var0-P0Fixing}
\begin{tabular}{c}
$I=40$\\
\\
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_7MOODCla5210_Special10_Var0-P0Fixing/res-I40-Phi}\\
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_7MOODCla5210_Special10_Var0-P0Fixing/res-I40-PhiError}\\
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_7MOODCla5210_Special10_Var0-P0Fixing/res-I40-Res}\\
\end{tabular}
\end{frame}


==> exL/ex3_I=40/out_TMeuler_7MOODNew5210_Special10_Var0-P0/TableConvs.tex <==
\begin{frame}
\frametitle{Linear | ex3 | convergence tables}
\captionsetup{labelformat=empty}
\tiny\setlength{\tabcolsep}{1pt}
\begin{table}[h]\centering
\caption{ex3 | MOODNew5210Special10 | Var0-P0}
\begin{tabular}{@{}ccccccccccccccccccccc@{}}\toprule
$I$ & \multicolumn{4}{l}{$P=0,1,2,5$} & & \multicolumn{4}{l}{$P=1,2,5$} & & \multicolumn{4}{l}{$P=2,5$} & & \multicolumn{4}{l}{$P=5$} & 5-CPD \\\cline{2-5}\cline{7-10}\cline{12-15}\cline{17-20}
& $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & 
\\\midrule
40 & 4.4E$-$04 & --- & 8.4E$-$03 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & 240 \\
\bottomrule
\end{tabular}
\end{table}

\end{frame}


==> exL/ex3_I=40/out_TMeuler_7MOODNew5210_Special10_Var0-P0/TablePlots.tex <==
\begin{frame}
\frametitle{Linear | ex3 | MOODNew5210Special10 | Var0-P0}
\begin{tabular}{c}
$I=40$\\
\\
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_7MOODNew5210_Special10_Var0-P0/res-I40-4MOOD-Phi}\\
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_7MOODNew5210_Special10_Var0-P0/res-I40-4MOOD-PhiError}\\
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_7MOODNew5210_Special10_Var0-P0/res-I40-4MOOD-Res}\\
\end{tabular}
\end{frame}


==> exL/ex3_I=40/out_TMeuler_7MOODNew5210_Special10_Var0-P0/iMOOD/Detail-I40.tex <==
\begin{frame}
\frametitle{Linear | ex3 | MOODNew5210Special10 | Var0-P0 | $I=40$}
\begin{tabular}{cccc}
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_7MOODNew5210_Special10_Var0-P0/iMOOD/res-I40-1MOOD-Phi} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_7MOODNew5210_Special10_Var0-P0/iMOOD/res-I40-2MOOD-Phi} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_7MOODNew5210_Special10_Var0-P0/iMOOD/res-I40-3MOOD-Phi} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_7MOODNew5210_Special10_Var0-P0/iMOOD/res-I40-4MOOD-Phi} \\
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_7MOODNew5210_Special10_Var0-P0/iMOOD/res-I40-1MOOD-PhiError} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_7MOODNew5210_Special10_Var0-P0/iMOOD/res-I40-2MOOD-PhiError} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_7MOODNew5210_Special10_Var0-P0/iMOOD/res-I40-3MOOD-PhiError} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_7MOODNew5210_Special10_Var0-P0/iMOOD/res-I40-4MOOD-PhiError} \\
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_7MOODNew5210_Special10_Var0-P0/iMOOD/res-I40-1MOOD-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_7MOODNew5210_Special10_Var0-P0/iMOOD/res-I40-2MOOD-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_7MOODNew5210_Special10_Var0-P0/iMOOD/res-I40-3MOOD-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_7MOODNew5210_Special10_Var0-P0/iMOOD/res-I40-4MOOD-Res} \\
\end{tabular}
\end{frame}


==> exL/ex3_I=40/out_TMeuler_8DSv1Cla5210_Special10_Var0-MOODFixing/TableConvs.tex <==
\begin{frame}
\frametitle{Linear | ex3 | convergence tables}
\captionsetup{labelformat=empty}
\tiny\setlength{\tabcolsep}{1pt}
\begin{table}[h]\centering
\caption{ex3 | DSv1Cla5210Special10 | Var0-MOODFixing}
\begin{tabular}{@{}ccccccccccccccccccccc@{}}\toprule
$I$ & \multicolumn{4}{l}{$P=0,1,2,5$} & & \multicolumn{4}{l}{$P=1,2,5$} & & \multicolumn{4}{l}{$P=2,5$} & & \multicolumn{4}{l}{$P=5$} & 5-CPD \\\cline{2-5}\cline{7-10}\cline{12-15}\cline{17-20}
& $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & 
\\\midrule
40 & 2.9E$-$04 & --- & 4.6E$-$03 & --- & & 1.9E$-$04 & --- & 4.6E$-$03 & --- & & 1.9E$-$04 & --- & 4.6E$-$03 & --- & & 1.9E$-$04 & --- & 4.6E$-$03 & --- & 10 \\
\bottomrule
\end{tabular}
\end{table}

\end{frame}


==> exL/ex3_I=40/out_TMeuler_8DSv1Cla5210_Special10_Var0-MOODFixing/TablePlots.tex <==
\begin{frame}
\frametitle{Linear | ex3 | DSv1Cla5210Special10 | Var0-MOODFixing}
\begin{tabular}{c}
$I=40$\\
\\
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_8DSv1Cla5210_Special10_Var0-MOODFixing/res-I40-Phi}\\
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_8DSv1Cla5210_Special10_Var0-MOODFixing/res-I40-PhiError}\\
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_8DSv1Cla5210_Special10_Var0-MOODFixing/res-I40-Res}\\
\end{tabular}
\end{frame}


==> exL/ex3_I=40/out_TMeuler_8DSv1New5210_Special10_Var0-MOOD/TableConvs.tex <==
\begin{frame}
\frametitle{Linear | ex3 | convergence tables}
\captionsetup{labelformat=empty}
\tiny\setlength{\tabcolsep}{1pt}
\begin{table}[h]\centering
\caption{ex3 | DSv1New5210Special10 | Var0-MOOD}
\begin{tabular}{@{}ccccccccccccccccccccc@{}}\toprule
$I$ & \multicolumn{4}{l}{$P=0,1,2,5$} & & \multicolumn{4}{l}{$P=1,2,5$} & & \multicolumn{4}{l}{$P=2,5$} & & \multicolumn{4}{l}{$P=5$} & 5-CPD \\\cline{2-5}\cline{7-10}\cline{12-15}\cline{17-20}
& $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$ & 
\\\midrule
40 & 2.7E$-$04 & --- & 4.6E$-$03 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & & 0 & --- & 0 & --- & 240 \\
\bottomrule
\end{tabular}
\end{table}

\end{frame}


==> exL/ex3_I=40/out_TMeuler_8DSv1New5210_Special10_Var0-MOOD/TablePlots.tex <==
\begin{frame}
\frametitle{Linear | ex3 | DSv1New5210Special10 | Var0-MOOD}
\begin{tabular}{c}
$I=40$\\
\\
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_8DSv1New5210_Special10_Var0-MOOD/res-I40-8DS-Phi}\\
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_8DSv1New5210_Special10_Var0-MOOD/res-I40-8DS-PhiError}\\
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_8DSv1New5210_Special10_Var0-MOOD/res-I40-8DS-Res}\\
\end{tabular}
\end{frame}


==> exL/ex3_I=40/out_TMeuler_8DSv1New5210_Special10_Var0-MOOD/iMOOD/Detail-I40.tex <==
\begin{frame}
\frametitle{Linear | ex3 | DSv1New5210Special10 | Var0-MOOD | $I=40$}
\begin{tabular}{cccc}
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_8DSv1New5210_Special10_Var0-MOOD/iMOOD/res-I40-5DS-Phi} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_8DSv1New5210_Special10_Var0-MOOD/iMOOD/res-I40-6DS-Phi} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_8DSv1New5210_Special10_Var0-MOOD/iMOOD/res-I40-7DS-Phi} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_8DSv1New5210_Special10_Var0-MOOD/iMOOD/res-I40-8DS-Phi} \\
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_8DSv1New5210_Special10_Var0-MOOD/iMOOD/res-I40-5DS-PhiError} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_8DSv1New5210_Special10_Var0-MOOD/iMOOD/res-I40-6DS-PhiError} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_8DSv1New5210_Special10_Var0-MOOD/iMOOD/res-I40-7DS-PhiError} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_8DSv1New5210_Special10_Var0-MOOD/iMOOD/res-I40-8DS-PhiError} \\
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_8DSv1New5210_Special10_Var0-MOOD/iMOOD/res-I40-5DS-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_8DSv1New5210_Special10_Var0-MOOD/iMOOD/res-I40-6DS-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_8DSv1New5210_Special10_Var0-MOOD/iMOOD/res-I40-7DS-Res} & 
\includegraphics[width=0.25\textwidth]{../../examplesL/ex3/out_TMeuler_8DSv1New5210_Special10_Var0-MOOD/iMOOD/res-I40-8DS-Res} \\
\end{tabular}
\end{frame}


==> sec5-numerics2.tex <==
\section{Numerical results} \label{sec:numerics}

Numerical experiments are carried out with the MOOD+AS scheme to give evidences of the method efficiency, namely to provide better accuracy still preserving the robustness. We detail three relevant problems that cover a large spectrum of application. The linear advection equation with a regular and a non-differential velocity is a classical building block in numerous problems. Next we analyse the method for the well-known B\"urgers equation involving a simple non-linearity. At last, we deal with the Euler system that represents the standard vector-valued non-linear hyperbolic system. 

To assess the error and convergence rate, we use the $L^1$ and $L^\infty$ errors given by
\begin{equation}
\label{eq:err_norms}
E_1 \equiv E_1(\Phi,I)=\Sum_{i=1}^{I} |\phi_i-\phi_i^{\text{ex}}| h,
\qquad
E_{\infty}\equiv E_\infty(\Phi,I) =\displaystyle\max_{i=1}^{I} |\phi_i-\phi_i^{\text{ex}}|.
\end{equation}
We further define the rate of convergence between two solutions/meshes $(\Phi_k,I_k)$, for $k=1,2$ where $I_1<I_2$ as
\begin{equation}
\label{eq:err_rates}
\mathcal{O}_{\alpha} \equiv \mathcal{O}_{\alpha} \left( (\Phi_1,I_1);(\Phi_2,I_2) \right) = 
\frac{|\log E_\alpha(\Phi_1,I_1)/E_\alpha(\Phi_2,I_2)|}{|\log I_1/I_2|}, \qquad
\alpha=1,\infty.
\end{equation}

The dynamical stencil strategy implies that one has to characterize the cells' position belonging to the stencil regarded from the reference cell where we evaluate the polynomial reconstruction. Table~\ref{colors_notation} gives the color codes used in the CPD map representations to distinguish 
%centered and shifted 
different stencils. For example, a centered stencil (same number of $\circ$ cells on the left and right side of the reference cell marked by a $\times$) is colored in green while a full left upwind stencil (all the cells are on the left side) is colored in violet. Obviously the colors' code also depends on the polynomial degree of the reconstruction.

\begin{table}[h]\centering
\caption{Colors notation for stencils.}
\label{colors_notation}
\begin{tabular}{@{}ccccc@{}}\toprule
$d$ & $\# S_i$ & $l$ & $r$ & \\\midrule
1 & 2 & 2 & 0 & OO\textcolor{blue}{X}\textcolor{white}{O}\textcolor{white}{O}\\
   &   & 1 & 1 & \textcolor{white}{O}O\textcolor{green}{X}O\textcolor{white}{O}\\
   &   & 0 & 2 & \textcolor{white}{O}\textcolor{white}{O}\textcolor{yellow}{X}OO\\\midrule
2 & 2 & 2 & 0 & OO\textcolor{blue}{X}\textcolor{white}{O}\textcolor{white}{O}\\
   &   & 1 & 1 & \textcolor{white}{O}O\textcolor{green}{X}O\textcolor{white}{O}\\
   &   & 0 & 2 & \textcolor{white}{O}\textcolor{white}{O}\textcolor{yellow}{X}OO\\\midrule
5 & 6 & 6 & 0 & OOOOOO\textcolor{violet}{X}\textcolor{white}{O}\textcolor{white}{O}\textcolor{white}{O}\textcolor{white}{O}\textcolor{white}{O}\textcolor{white}{O}\\
   &   & 5 & 1 & \textcolor{white}{O}OOOOO\textcolor{indigo}{X}O\textcolor{white}{O}\textcolor{white}{O}\textcolor{white}{O}\textcolor{white}{O}\textcolor{white}{O}\\
   &   & 4 & 2 & \textcolor{white}{O}\textcolor{white}{O}OOOO\textcolor{blue}{X}OO\textcolor{white}{O}\textcolor{white}{O}\textcolor{white}{O}\textcolor{white}{O}\\
   &   & 3 & 3 & \textcolor{white}{O}\textcolor{white}{O}\textcolor{white}{O}OOO\textcolor{green}{X}OOO\textcolor{white}{O}\textcolor{white}{O}\textcolor{white}{O}\\
   &   & 2 & 4 & \textcolor{white}{O}\textcolor{white}{O}\textcolor{white}{O}\textcolor{white}{O}OO\textcolor{yellow}{X}OOOO\textcolor{white}{O}\textcolor{white}{O}\\
   &   & 1 & 5 & \textcolor{white}{O}\textcolor{white}{O}\textcolor{white}{O}\textcolor{white}{O}\textcolor{white}{O}O\textcolor{orange}{X}OOOOO\textcolor{white}{O}\\
   &   & 0 & 6 & \textcolor{white}{O}\textcolor{white}{O}\textcolor{white}{O}\textcolor{white}{O}\textcolor{white}{O}\textcolor{white}{O}\textcolor{red}{X}OOOOOO\\\bottomrule
\end{tabular}
\end{table}


\subsection{Advection equation} \label{ssec:advection}

The scalar linear convective steady-state problem reads
\begin{equation}
\frac{\textrm{d}}{\textrm{d}x}\Big (u(x)\phi(x)\Big)=S(x),\quad x\in \Omega, \label{eq:linear}
\end{equation}
where $u\equiv u(x)>0$ is a given velocity function and Dirichlet boundary condition $\phi_{\text{L}}$ is prescribed on the left side of domain $\Omega$. Since $u$ may present some irregularities, the solution is not necessarily smooth enough to perform all the polynomial reconstructions with $d^{\max}$ hence the CPD and CS maps must be adapted accordingly.

The numerical flux $\mathcal F(\phi_{i+\frac{1}{2},-},\phi_{i+\frac{1}{2},+};x_{i+\frac{1}{2}})$ is the classical upwind one.
For given CPD and CS maps $\mathcal M, \mathcal S$, and noticing that the problem $\mathcal{G}(\Phi, \mathcal M, \mathcal S)=0$ is affine, we use a Gauss-type procedure to nullify the residual.
% Chain detector and cascade
Next, the chain detector associated to this linear equation follows the chain: ED, PD, LOD, and SD where all these detectors have been defined in the previous section (see also \cite{1D_SS}). 
%--- F I G ------
\begin{figure}
	\begin{center}
		\begin{tabular}{cc}
			\includegraphics[width=0.4\textwidth]{figures/exact_linear_regular} &
			\includegraphics[width=0.4\textwidth]{figures/exact_linear_irregular}
		\end{tabular}
		\caption{ \label{fig:ex_sol_linear} Exact solutions (black) 
			and associate velocities (red) for the linear equation on $\overline\Omega=[0;1]$ --- 
			$\phi(x)=1/u(x)$ ---
			Left: regular solution $u(x)= 2 \sin(2\pi x) + 3$ --- 
			Right: irregular solution $u(x)=x+2, \; \text{if} \;  x<1/2$ or $u(x)=50(x-1/2)+5/2$, otherwise.}
	\end{center}
\end{figure}
%--- F I G ------


\subsubsection{Regular solution}
A regular situation is achieved with the smooth velocity function $u(x)= 2 \sin(2\pi x) + 3$ leading to the solution depicted in Fig.~\ref{fig:ex_sol_linear} on left panel. The boundary conditions are set to $1/3$ at $x=0$ and an outflow condition at $x=1$.
In table~\ref{tab:conv_ex1} one reports the $L_1$ and  $L_\infty$ errors, together with the convergence rates for a 6th order MOOD scheme. Optimal orders \textcolor{red}{RAPH: in fact the rates are not optimal for TM1 and TM2 I read 5.2, 5.5 which is good but not optimal.} are obtained using the three solvers: Linear and Time Marching TM1, TM2 schemes using the  first-, second-, and sixth-order accurate reconstructions.
\textcolor{red}{Only the sixth-order scheme results are reported here.}

\begin{table}[h]
\setlength\tabcolsep{3 pt}
{\tablepolice
\centering
\caption{Advection with regular velocity: errors and convergence rate. L solver (left), TM1 solver (middle), TM2 solver (right)}
\label{tab:conv_ex1}
\begin{tabular}{@{}cccccccc@{}}\toprule
$I$ & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$\\\midrule
40 & 1.1E$-$05 & --- & 6.9E$-$05 & --- \\
80 & 1.7E$-$07 & 6.0 & 1.4E$-$06 & 5.6 \\
160 & 2.6E$-$09 & 6.0 & 2.4E$-$08 & 5.9\\\bottomrule
\end{tabular}
\hskip 2em
\begin{tabular}{@{}cccccccc@{}}\toprule
$I$ & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$\\\midrule
40 & 1.1E$-$05 & --- & 6.6E$-$05 & --- \\
80 & 2.3E$-$07 & 5.5 & 1.8E$-$06 & 5.2 \\
160 & 6.2E$-$09 & 5.2 & 3.8E$-$08 & 5.5 \\\bottomrule
\end{tabular}
\hskip 2em
\begin{tabular}{@{}cccccccc@{}}\toprule
$I$ & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$\\\midrule
40 & 1.1E$-$05 & --- & 6.6E$-$05 & --- \\
80 & 2.3E$-$07 & 5.5 & 1.8E$-$06 & 5.2 \\
160 & 6.2E$-$09 & 5.2 & 3.8E$-$08 & 5.5 \\\bottomrule
\end{tabular}
}
\end{table}


%\begin{table}[h]\centering
%\caption{Advection example 1 (regular) | MOOD | TM1 solver (the initial solution is the $\mathbb{P}_0$ solution with linear BC %initial solution): convergence table.}
%\label{tab:L_ex1_TM1}
%\begin{tabular}{@{}cccccccc@{}}\toprule
%$I$ & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$\\\midrule
%40 & 1.1E$-$05 & --- & 6.6E$-$05 & --- \\
%80 & 2.3E$-$07 & 5.5 & 1.8E$-$06 & 5.2 \\
%160 & 6.2E$-$09 & 5.2 & 3.8E$-$08 & 5.5 \\\bottomrule
%\end{tabular}
%\end{table}


%\begin{table}[h]\centering
%\caption{Advection example 1 (regular) | MOOD | TM2 solver (the initial solution is the $\mathbb{P}_0$ solution with linear BC %initial solution): convergence table.}
%\label{tab:L_ex1_TM2}
%\begin{tabular}{@{}cccccccc@{}}\toprule
%$I$ & $E_1$ & ${\mathcal O}_1$ & $E_\infty$ & ${\mathcal O}_\infty$\\\midrule
%40 & 1.1E$-$05 & --- & 6.6E$-$05 & --- \\
%80 & 2.3E$-$07 & 5.5 & 1.8E$-$06 & 5.2 \\
%160 & 6.2E$-$09 & 5.2 & 3.8E$-$08 & 5.5 \\\bottomrule
%\end{tabular}
%\end{table}

Moreover Fig.~\ref{fig:L_ex1_L} presents the numerical solutions (left panel), the CPD maps (middle panel), and $L_1$ errors (right panel) for L scheme using the 6th-order MOOD algorithm. We observe that the Cell Polynomial Degree is maintained at its maximum leading to the optimal accuracy. No oscillation is detected. We do not present the TM1, and TM2 figures since they are almost similar to the L one.

\begin{table}[h]\centering
\caption{Advection example 1 (regular) | MOOD | L solver: exact and numerical solutions for $I=40$ (left), CPD map for $I=40$ (center), and errors for $I=40$/black, $I=80$/red, and $I=160$/green (right).
\textcolor{red}{RAPH: I propose to enlarge the figure to fill the width entirely playing with hspace to fit them, like here. The problem is due to white spaces around the figures. Another option is to postprocess the figures from matlab and crop the spaces} }
\label{fig:L_ex1_L}
\begin{tabular}{ccc}
\hspace{-0.75cm}
\includegraphics[width=0.37\textwidth]{exL/exL_ex1_LSgauss_7MOODNew5210_article/res-I40-1MOOD-Phi_article} &
\hspace{-0.75cm}
\includegraphics[width=0.37\textwidth]{exL/exL_ex1_LSgauss_7MOODNew5210_article/res-I40-1MOOD-Phi_CPD_article} &
\hspace{-0.75cm}
\includegraphics[width=0.37\textwidth]{exL/exL_ex1_LSgauss_7MOODNew5210_article/errors_article}
\end{tabular}
\end{table}


%\begin{table}[h]\centering
%\caption{Advection example 1 (regular) | MOOD | TM1 solver (the initial solution is the $\mathbb{P}_0$ solution with linear BC initial solution): exact and numerical solutions for $I=40$ (left), CPD map for $I=40$ (center), and errors for $I=40$/black, $I=80$/red, and $I=160$/green (right).}
%\label{fig:L_ex1_TM1}
%\begin{tabular}{ccc}
%\includegraphics[width=0.31\textwidth]{exL/exL_ex1_TMeuler_7MOODCla5210_Special10_Var0-P0_article/res-I40-Phi_article} &
%\includegraphics[width=0.31\textwidth]{exL/exL_ex1_TMeuler_7MOODCla5210_Special10_Var0-P0_article/res-I40-Phi_CPD_article} &
%\includegraphics[width=0.31\textwidth]{exL/exL_ex1_TMeuler_7MOODCla5210_Special10_Var0-P0_article/errors_article}
%\end{tabular}
%\end{table}


%\begin{table}[h]\centering
%\caption{Advection example 1 (regular) | MOOD | TM2 solver (the initial solution is the $\mathbb{P}_0$ solution with linear BC initial solution): exact and numerical solutions for $I=40$ (left), CPD map for $I=40$ (center), and errors for $I=40$/black, $I=80$/red, and $I=160$/green (right).}
%\label{fig:L_ex1_TM2}
%\begin{tabular}{ccc}
%\includegraphics[width=0.31\textwidth]{exL/exL_ex1_TMeuler_7MOODNew5210_Special10_Var0-P0_article/res-I40-1MOOD-Phi_article} &
%\includegraphics[width=0.31\textwidth]{exL/exL_ex1_TMeuler_7MOODNew5210_Special10_Var0-P0_article/res-I40-1MOOD-Phi_CPD_article} &
%\includegraphics[width=0.31\textwidth]{exL/exL_ex1_TMeuler_7MOODNew5210_Special10_Var0-P0_article/errors_article}
%\end{tabular}
%\end{table}


\subsubsection{Irregular solution}
The second test is dedicated to the situation with a rough velocity given by 
\[
u(x) =
\begin{cases} 
x+2,           & \text{if $x\in[0;1/2]$},\\
50(x-1/2)+5/2, & \text{if $x\in[1/2;1]$},
\end{cases} 
\]
leading to the solution depicted in Fig.~\ref{fig:ex_sol_linear} on right panel.
This solution is continuous but not differential at location $x=1/2$.
The boundary conditions are set to $1/2$ at $x=0$ and an outflow condition at $x=1$.

\begin{table}[ht]\centering
\caption{Advection example 2 (irregular) | L solver: exact and numerical solutions (left), CPD map (center), and errors (right) for $I=40$ --- top/MOOD, bottom/AS.}
\label{fig:L_ex2_L}
\begin{tabular}{ccc}
\includegraphics[width=0.31\textwidth]{exL/exL_ex3_LSgauss_7MOODNew5210_article/res-I40-4MOOD-Phi_article} &
\includegraphics[width=0.31\textwidth]{exL/exL_ex3_LSgauss_7MOODNew5210_article/res-I40-4MOOD-Phi_CPD_article} &
\includegraphics[width=0.31\textwidth]{exL/exL_ex3_LSgauss_7MOODNew5210_article/res-I40-4MOOD-PhiError_article}\\
\includegraphics[width=0.31\textwidth]{exL/exL_ex3_LSgauss_8DSv1New5210_article/res-I40-8DS-Phi_article} &
\includegraphics[width=0.31\textwidth]{exL/exL_ex3_LSgauss_8DSv1New5210_article/res-I40-8DS-Phi_CPD_article} &
\includegraphics[width=0.31\textwidth]{exL/exL_ex3_LSgauss_8DSv1New5210_article/res-I40-8DS-PhiError_article}
\end{tabular}
\end{table}

Unlimited reconstructions, \textit{i.e.} using the systematic $\mathbb P_5$ polynomial representation, provides a non-physical solution and spurious oscillations are generated. To remove the overshooting, the original MOOD \textit{a posteriori} strategy (Static Stencil) is applied by reducing the polynomial degree for the cells that require a cure. We recall that the stencils are centered with respect to the reference cell leading to a strong cut of the degree in the vicinity of a shock. The alternative Dynamical Stencil method we propose modifies the stencil structure in order to catch the neighbor cells that enjoy a high degree of reconstruction that helps to maintain the optimal accuracy.  

We present in Fig.~\ref{fig:L_ex2_L} the two strategies and their consequences for the accuracy and stability. The first row display the curve, CPD map and errors using the Static Stencil (the original MOOD method) whereas the second row display the same figures for the Dynamical Stencil strategies. In both case, the stability is achieved and no oscillations are reported. The CPD map configurations are different since the Dynamical Stencil only suffer of two degree reduction cells. We notice the stencil upwinding close to the singularities in accordance with the relative position (left upwind on the left side and right upwind on the right side). The last column depicts the error values, cell by cell, and show the dramatic improvement of the accuracy.     

We have carried out the same simulation with the two Time Marching strategies we reproduce in Figs~\ref{fig:L_ex2_TM1}, and \ref{fig:L_ex2_TM2} for TM1 and TM2 respectively. Curiously, the TM1 strategy produce a better CPD map in the case of a Static Stencil and produce a slightly better solution. The TM2 method exactly provides the same CPD map that the L method and, once again, the Dynamical Stencil strategy achieve a good improvement of the polynomial reconstruction by choosing the best stencil. 



\begin{table}[ht]\centering
\caption{Advection example 2 (irregular) | TM1 solver: exact and numerical solutions (left), CPD map (center), and errors (right) for $I=40$ --- top/MOOD (the initial solution is the $\mathbb{P}_0$ solution with linear BC initial solution), bottom/AS (the initial solution is the MOOD solution).}
\label{fig:L_ex2_TM1}
\begin{tabular}{ccc}
\includegraphics[width=0.31\textwidth]{exL/exL_ex3_TMeuler_7MOODCla5210_Special10_Var0-P0Fixing_article/res-I40-Phi_article} &
\includegraphics[width=0.31\textwidth]{exL/exL_ex3_TMeuler_7MOODCla5210_Special10_Var0-P0Fixing_article/res-I40-Phi_CPD_article} &
\includegraphics[width=0.31\textwidth]{exL/exL_ex3_TMeuler_7MOODCla5210_Special10_Var0-P0Fixing_article/res-I40-PhiError_article}\\
\includegraphics[width=0.31\textwidth]{exL/exL_ex3_TMeuler_8DSv1Cla5210_Special10_Var0-MOODFixing_article/res-I40-Phi_article} &
\includegraphics[width=0.31\textwidth]{exL/exL_ex3_TMeuler_8DSv1Cla5210_Special10_Var0-MOODFixing_article/res-I40-Phi_CPD_article} &
\includegraphics[width=0.31\textwidth]{exL/exL_ex3_TMeuler_8DSv1Cla5210_Special10_Var0-MOODFixing_article/res-I40-PhiError_article}
\end{tabular}
\end{table}

\begin{table}[ht]\centering
\caption{Advection example 2 (irregular) | TM2 solver: exact and numerical solutions (left), CPD map (center), and errors (right) for $I=40$ --- top/MOOD (the initial solution is the $\mathbb{P}_0$ solution with linear BC initial solution), bottom/AS (the initial solution is the MOOD solution).}
\label{fig:L_ex2_TM2}
\begin{tabular}{ccc}
\includegraphics[width=0.31\textwidth]{exL/exL_ex3_TMeuler_7MOODNew5210_Special10_Var0-P0_article/res-I40-4MOOD-Phi_article} &
\includegraphics[width=0.31\textwidth]{exL/exL_ex3_TMeuler_7MOODNew5210_Special10_Var0-P0_article/res-I40-4MOOD-Phi_CPD_article} &
\includegraphics[width=0.31\textwidth]{exL/exL_ex3_TMeuler_7MOODNew5210_Special10_Var0-P0_article/res-I40-4MOOD-PhiError_article}\\
\includegraphics[width=0.31\textwidth]{exL/exL_ex3_TMeuler_8DSv1New5210_Special10_Var0-MOOD_article/res-I40-8DS-Phi_article} &
\includegraphics[width=0.31\textwidth]{exL/exL_ex3_TMeuler_8DSv1New5210_Special10_Var0-MOOD_article/res-I40-8DS-Phi_CPD_article} &
\includegraphics[width=0.31\textwidth]{exL/exL_ex3_TMeuler_8DSv1New5210_Special10_Var0-MOOD_article/res-I40-8DS-PhiError_article}
\end{tabular}
\end{table}

\newpage
\subsection{Burgers' equation} \label{ssec:burgers}

Inviscid Burgers steady-state problem is an attractive benchmark since we are dealing with a simple scalar non-linear model which may nonetheless generate discontinuous solutions, it reads
\[
\frac{\text{d}}{\text{d}x}\Big(\frac{\phi^2}{2}\Big)=S(x),\quad x\in \Omega,
\]
where $S\equiv S(x)$ is a given source term.
Dirichlet boundary conditions $\phi_{\text{L}}$ and $\phi_{\text{D}}$ are prescribed on the left and right boundaries of $\Omega$, respectively.

The numerical benchmark is the following (\cite{burgers_ex_irregular}):
\[
\begin{cases}
\frac{\partial\phi}{\partial t}+\frac{\partial}{\partial x}\Big(\frac{\phi^2}{2}\Big)=\sin(x)\cos(x), & x\in [0,\pi],\\
\phi(x,0)=\beta\sin(x), & x\in [0,\pi],\\
\phi(0,t)=\phi(\pi,t)=0, & t\in\mathds{R},
\end{cases}
\]
whose steady-state solution is
\begin{itemize}
\item if $\beta\in]-\infty,-1]$: $\phi(x,\infty)=\sin(x)$;
\item if $\beta\in]-1,1[$: $\phi(x,\infty)=\begin{cases}\sin(x), & \text{if } x\in[0,x^\ast[\\-\sin(x), & \text{if } x\in[x^\ast,\pi],\end{cases}$
with $x^\ast=\pi-\arcsin\left(\sqrt{1-\beta^2}\right)$;
\item if $\beta\in[1,\infty[$: $\phi(x,\infty)=-\sin(x)$.
\end{itemize}

Note that the location of the shock is determined by parameter $\beta$ through conservation of mass 
$$
\int_0^\pi\phi(x,t)\,\text{d}x=\int_0^\pi\beta\sin(x)\,\text{d}x=2\beta.
$$ 
In our case we take $x^\ast=\frac{3\pi}{4}$, which implies $\beta=\frac{\sqrt{2}}{2}$.

The numerical flux $\mathcal F(\phi_{i+\frac{1}{2},-},\phi_{i+\frac{1}{2},+};x_{i+\frac{1}{2}})$ is the Rusanov one, that is,
\[
\mathcal{F}(\phi_{i+\frac{1}{2},-},\phi_{i+\frac{1}{2},+};x_{i+\frac{1}{2}})=\frac{1}{2}\left(\frac{\phi_{i+\frac{1}{2},-}^2}{2}+\frac{\phi_{i+\frac{1}{2},+}^2}{2}\right)-\lambda_{i+\frac{1}{2}}(\phi_{i+\frac{1}{2},+}-\phi_{i+\frac{1}{2},-}),
\]
where $\lambda_{i+\frac{1}{2}}=\max(|\phi_i|,|\phi_{i+1}|)$, and the linear problem detector chain is used.

The first simulation has been carried out with the original MOOD method using the Static Stencil (first row in Fig~\ref{fig:burger_benchmark}) whereas we present, in the second row, the Dynamical Stencil reconstruction to improve the accuracy by preserving the high degree of the polynomial reconstruction. We note that no oscillations have been created in the both cases. The CPD map with the colors' code indicate that the Dynamical Stencil strategy manage to recover the optimal degree by smartly upwinding the stencils. The last column confirms the spectacular gain where the error is lower of several magnitudes in the shock vicinity. The chief point is an excellent improvement of the solution quality where regular. 
\begin{table}[h]\label{fig:burger_benchmark}
\centering
\caption{Burgers example | NL solver: exact and numerical solutions (left), CPD map (center), and errors (right) for $I=40$ --- top/MOOD (the initial solution is the $\mathbb{P}_0$ solution with linear BC initial solution), bottom/AS (the initial solution is the MOOD solution).}
\begin{tabular}{ccc}
\includegraphics[width=0.31\textwidth]{exB/out_NLSfsolveV3_7MOODNew5210_Var0-P0_article/res-I40-3MOOD-Phi_article} &
\includegraphics[width=0.31\textwidth]{exB/out_NLSfsolveV3_7MOODNew5210_Var0-P0_article/res-I40-3MOOD-CPD_article} &
\includegraphics[width=0.31\textwidth]{exB/out_NLSfsolveV3_7MOODNew5210_Var0-P0_article/res-I40-3MOOD-PhiError_article}\\
\includegraphics[width=0.31\textwidth]{exB/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD_article/res-I40-4DS-Phi_article} &
\includegraphics[width=0.31\textwidth]{exB/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD_article/res-I40-4DS-CPD_article} &
\includegraphics[width=0.31\textwidth]{exB/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD_article/res-I40-4DS-PhiError_article}
\end{tabular}
\end{table}

We draw similar conclusions with the TM1 and TM2 method and display in Figs~\ref{fig:burger_benchmark_TM1}-\ref{fig:burger_benchmark_TM2} the approximated solution, the CPD map together with the colors'' code and the errors.

\begin{table}[h]\label{fig:burger_benchmark_TM1}\centering
\caption{Burgers example | TM1 solver: exact and numerical solutions (left), CPD map (center), and errors (right) for $I=40$ --- top/MOOD (the initial solution is the $\mathbb{P}_0$ solution with linear BC initial solution), bottom/AS (the initial solution is the MOOD solution).}
\begin{tabular}{ccc}
\includegraphics[width=0.31\textwidth]{exB/out_TMeuler_7MOODCla5210_Var0-P0Fixing_article/res-I40-Phi_article} &
\includegraphics[width=0.31\textwidth]{exB/out_TMeuler_7MOODCla5210_Var0-P0Fixing_article/res-I40-CPD_article} &
\includegraphics[width=0.31\textwidth]{exB/out_TMeuler_7MOODCla5210_Var0-P0Fixing_article/res-I40-PhiError_article}\\
\includegraphics[width=0.31\textwidth]{exB/out_TMeuler_8DSv1Cla5210_Var0-MOODFixing_article/res-I40-Phi_article} &
\includegraphics[width=0.31\textwidth]{exB/out_TMeuler_8DSv1Cla5210_Var0-MOODFixing_article/res-I40-CPD_article} &
\includegraphics[width=0.31\textwidth]{exB/out_TMeuler_8DSv1Cla5210_Var0-MOODFixing_article/res-I40-PhiError_article}
\end{tabular}
\end{table}

\begin{table}[h]\label{fig:burger_benchmark_TM2}\centering
\caption{Burgers example | TM2 solver: exact and numerical solutions (left), CPD map (center), and errors (right) for $I=40$ --- top/MOOD (the initial solution is the $\mathbb{P}_0$ solution with linear BC initial solution), bottom/AS (the initial solution is the MOOD solution).}
\begin{tabular}{ccc}
\includegraphics[width=0.31\textwidth]{exB/out_TMeuler_7MOODNew5210_Var0-P0_article/res-I40-3MOOD-Phi_article} &
\includegraphics[width=0.31\textwidth]{exB/out_TMeuler_7MOODNew5210_Var0-P0_article/res-I40-3MOOD-CPD_article} &
\includegraphics[width=0.31\textwidth]{exB/out_TMeuler_7MOODNew5210_Var0-P0_article/res-I40-3MOOD-PhiError_article}\\
\includegraphics[width=0.31\textwidth]{exB/out_TMeuler_8DSv1New5210_Var0-MOOD_article/res-I40-4DS-Phi_article} &
\includegraphics[width=0.31\textwidth]{exB/out_TMeuler_8DSv1New5210_Var0-MOOD_article/res-I40-4DS-CPD_article} &
\includegraphics[width=0.31\textwidth]{exB/out_TMeuler_8DSv1New5210_Var0-MOOD_article/res-I40-4DS-PhiError_article}
\end{tabular}
\end{table}

\newpage 
\subsection{Euler system of equations} \label{ssec:euler}
Let $\bm{U}=(\rho,\rho u ,E)^T$ be the conservative quantities and  $\bm{V}(\rho,u,p)^T$, the vector of state variables density, velocity, and pressure. We seek a solution of the steady-state 1D Euler equations with source terms given by
\begin{equation}
\label{eq:Euler1D}
\frac{\textrm{d}\bm{F}(\bm{U})}{\textrm{d}x}=\bm{S}, \qquad\text{in }\Omega,
\end{equation}
where the flux vector is given by $\bm{F}(\bm{U})=(\rho u,\rho u^2+p,u(E+p))^T$ and the regular source vector term is given by $\bm{S}\equiv\bm{S}(x)=(\frac{\textrm{d}D}{\textrm{d}x},\frac{\textrm{d}F}{\textrm{d}x},\frac{\textrm{d}H}{\textrm{d}x})^T\equiv(\frac{\textrm{d}D}{\textrm{d}x}(x),\frac{\textrm{d}F}{\textrm{d}x}(x),\frac{\textrm{d}H}{\textrm{d}x}(x))^T$.
Total energy $E$, specific internal energy $e$, and sound-speed $a$ are expressed as
\begin{equation}
\label{eq:Eea}
E=\frac{1}{2}\rho u^2+\rho e, \quad
e=\frac{p}{\rho(\gamma-1)}, \quad
a=\sqrt{\frac{\gamma p}{\rho}},
\end{equation}
respectively, where $\gamma>1$ is the ratio of specific heat. System~\eqref{eq:Euler1D} is completed with Dirichlet boundary conditions
\[
\bm{V}(x_{\text{L}})=\bm{V}_\text{L}\equiv(\rho_\text{L},u_\text{L},p_\text{L})^T
\quad\text{ and }\quad
\bm{V}(x_{\text{R}})=\bm{V}_\text{R}\equiv(\rho_\text{R},u_\text{R},p_\text{R})^T.
\]


We deduce the algebraic system to be solved 
\begin{align}
	\label{eq:D}
	\rho u &= D,    \\
	\label{eq:F}
	\rho u^2+p &= F, \\
	\label{eq:H}
	u(E+p) &= H,\\
	\label{eq:E} 
	\frac{1}{2}\rho u^2+\frac{p}{\gamma-1}&=E.
\end{align}
Notice that $D$, $F$, and $H$ depend on additional constants we shall fix with the boundary conditions.
Analytic solutions for the steady-state problem are detailed in \cite{1D_SS}. 

\vskip 1em
Let us denote by $\bm{\mathcal U}=(\bm{U}_i)_{i=1,\ldots,I}$ the
$3\times I$ matrix containing the approximations of the mean-values for $\rho$, $\rho u$, and $E$ while
$\bm{\mathcal U}^k$ stands for the data associated to stage $k$. The numerical flux 
$\mathcal F (\bm{U}_-,\bm{U}_+;x)$ is chosen to be the HLL/HLLE one proposed in \cite{hll} where $\bm{U}_-$ and $\bm{U}_+$ are the left and right states at interface $x$
\[
\mathcal{F}(\bm{U}_-,\bm{U}_+;x)=
\begin{cases} 
\bm{U}_- & \text{if $s_-\geq 0$},\\
\frac{s_+\bm{F}(\bm{U}_-)-s_-\bm{F}(\bm{U}_+)+s_+s_-(\bm{U}_+-\bm{U}_-)}{s_+-s_-} & \text{if $s_-\leq 0 \leq s_+$} \, ,\\
\bm{U}_+ & \text{if $s_+\leq 0$},
\end{cases}
\]
where we take the numerical velocities $s_-=\min(u_--a_-,u_+-a_+)$ and $s_+=\max(u_-+a_-,u_++a_+)$ for the sake of simplicity. 
\begin{remI}
	Notice that such a flux does not strictly preserve the positivity of the density and pressure. If one requires a formally positivity preserving flux, the Rusanov flux, equipped with the adequate numerical velocity, should be used (see \cite{munz91} for question of positivity preservation).
\end{remI}

For given CPD and CS maps $\mathcal M^k,\mathcal S^k$, we introduce the nonlinear operator
\[
\bm{\mathcal U}\in\mathbb R^{3\times I}\to \mathcal{G}(\bm{\mathcal U},\mathcal M^k,\mathcal S^k) \in\mathbb R^{3\times I}
\]
and we seek for $\bm{\mathcal U}^{k+1}$ such that  $\mathcal{G}(\bm{\mathcal U}^{k+1},\mathcal M^k,\mathcal S^k)=0$.

%Again we consider either a nonlinear solver (NL) and the time-marching (TM) technique to solve this set of equations. 
%Notice that for the NL case, an additional condition is considered to fix the shock 
%position when dealing with two different regimes on the left and right boundaries.
%For the TM method, the initial condition for density imposes the position of the shock.
% detector chain and cascade
The detector chain associated to the Euler equation follows the chain depicted in Fig.~\ref{fig:chain_detector_euler}. Here the PAD box checks the positivity of density and pressure.
% --- FIG --- detector chain
\begin{figure}[ht]
	\centering
	\includegraphics[width=1.0\textwidth]{figures/chain_euler}
	\caption{Chain of detectors used for Euler system of equations
		to check if a cell value is valid and accepted, or, if it is discarded 
		and need to be recomputed after reduction of the local cell polynomial degree.
		PAD: Physical Admissible Detector,
		ED: Extrema Detector,
		PD: Plateau Detector,
		LOD: Local Oscillation Detector,
		SD: Smoothness Detector.
	}
	\label{fig:chain_detector_euler}
\end{figure}
% --- FIG ---
Because we consider only one polynomial degree per cell for each component of $\bm{\mathcal U}$ {\it i.e.} density, momentum and total energy, we determine only one polynomial degree map. Only the density variable is tested for the ED, LOD, and SD detection criteria and the CS map is determined accordingly.
The MOOD loop is escaped if $\mathcal{M}^{k+1}=\mathcal{M}^{k}$.

To assess the validity of the method, we consider the following data. The domain is given by $x_{\text{L}}=0$, $x_{\text{R}}=1$ and we take $D(x)=1$, $F(x)=0.027x + 0.6137$, and $H(x)=0.375$.  The first two conditions for the admissible space are trivially satisfied. The third condition, $\frac{DH}{F^2}\leq\frac{\gamma^2}{2(\gamma^2-1)}$ is also satisfied \cite{1D_SS}.
%\[
%\max_{x\in[0,1]}\frac{DH}{F^2}=\max_{x\in[0,1]}\frac{0.375}{(0.027x + 0.6137)^2}=0.9957\leq\frac{\gamma^2}{2(\gamma^2-1)}=1.0208.
%\]
The expressions for the supersonic solution and the subsonic solution branches are given by
\begin{gather} \label{eq:supsub}
	\rho_\textup{sup}(x)=0.126x - 3.3333\sqrt{1.96(0.027x + 0.6137)^2 - 0.72}+ 2.8639,\\
	\rho_\textup{sub}(x)=0.126x + 3.3333\sqrt{1.96(0.027x + 0.6137)^2 - 0.72}+ 2.8639,
\end{gather}
respectively and depicted in Fig.~\ref{fig:EulerrhoSupAndrhoSub}.
% --- FIG --- exact Euler figure
%   To create the fgure run gnuplot script in DATA/Euler/euler_ex.gnu
\begin{figure}[ht]
	\centering
	% \includegraphics[width=6cm]{figures/EulerrhoSupAndrhoSub}
	\includegraphics[width=0.5\textwidth]{figures/ex_Euler}
	\caption{Plots of the supersonic and subsonic branches $\rho_\textup{sup}$ (red) and $\rho_\textup{sub}$ (blue) from \eqref{eq:supsub},
		and the exact solution of the irregular density (shock located at $x=0.6$) employed in this paper (black).}
	\label{fig:EulerrhoSupAndrhoSub}
\end{figure}
% --- FIG ---
As mentioned in Remark \ref{rem:four_cases}, only three situations have to be considered. We have two regular situations when considering supersonic or subsonic states on both boundary points. The case where we prescribe subsonic state at the left boundary point and supersonic state at the right does not provide  an entropic solution and must be discarded. 
At last, prescribing supersonic state on the left boundary point and subsonic state on the right boundary produces a solution with a shock wave located at $x_\textup{c}$. We now present this last situation.

To enforce the shock position at $x_\textup{c}=0.6$, we set  
\begin{equation} \label{eq:constraintA}
A=
\int_{x_{\textup{L}}}^{x_{\textup{R}}} \rho^0(x)\,\textup{d}x=
%\int_{x_{\textup{L}}}^{x_{\textup{R}}} \left((\rho_\text{L}-\rho_\text{R})(1-x)^{0.4550}+\rho_\text{R}\right)\,\textup{d}x =
2.8975. 
\end{equation}
for an initial density profile 
\begin{equation}
\rho^0(x) = 
\begin{cases}
\rho_\text{L} & \text{ if $x\leq x_0=0.6873$} \\
\rho_\text{R} & \text{ otherwise} \\
\end{cases}
\end{equation}
where $x_0$ is determined by solving~\eqref{eq:constraintA} (different from $x_\textup{c}$). We initialize the other variables as $u^0=D/\rho^0$ and $p^0$ derives from relation \eqref{eq:F} and $E^0$ is deduced from relation \eqref{eq:E}. The exact solution for the density variable is depicted in black in Fig.~\ref{fig:EulerrhoSupAndrhoSub}.

In \cite{1D_SS} a numerical studied as been carried out to analyze the MOOD scheme behavior and we refer the reader to these results which can be summarized as follows:
\begin{itemize}
	\item the unlimited high order schemes produce oscillatory results;
	\item the MOOD scheme is able to mitigate those spurious oscillations by reducing the CPD map in the vicinity of the shock position. 
\end{itemize}


We compare in Table \ref{tab:euler_benchmark} the Static Stencil (first row) versus the Dynamical Stencil (second row) strategies. We just present the simulations carried out with the non-linear solver since the results are quite similar with the Time Marching method. The first column display the numerical solution for the two cases and no oscillations are reported. The CPD map associated with the colors'' code show that the dynamical stencil method enables to recover the full polynomial degree. In the last case, the stencil are shifted in order to avoid the cell that carries the discontinuity. Consequently, we achieve a very high accuracy in the domains where the solution is still regular while avoiding non-physical numerical artifacts. The error is cut by more than four magnitudes in the vicinity of the shock.
 
\begin{table}[h]\centering\label{tab:euler_benchmark}
\caption{Euler example | NL solver: exact and numerical solutions (left), CPD map (center), and errors (right) for $I=40$ (shock location at an interface) --- top/MOOD (the initial solution is the $\mathbb{P}_0$ solution with linear BC initial solution), bottom/AS (the initial solution is the MOOD solution).}
\begin{tabular}{ccc}
\includegraphics[width=0.31\textwidth]{exE/I40/out_NLSfsolveV3_7MOODNew5210_Var0-P0_article/res-I40-4MOOD-Rho_article} &
\includegraphics[width=0.31\textwidth]{exE/I40/out_NLSfsolveV3_7MOODNew5210_Var0-P0_article/res-I40-4MOOD-CPD_article} &
\includegraphics[width=0.31\textwidth]{exE/I40/out_NLSfsolveV3_7MOODNew5210_Var0-P0_article/res-I40-4MOOD-RhoError_article}\\
\includegraphics[width=0.31\textwidth]{exE/I40/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD_article/res-I40-8DS-Rho_article} &
\includegraphics[width=0.31\textwidth]{exE/I40/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD_article/res-I40-8DS-CPD_article} &
\includegraphics[width=0.31\textwidth]{exE/I40/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD_article/res-I40-8DS-RhoError_article}
\end{tabular}
\end{table}

\begin{table}[h]\centering
\caption{Euler example | NL solver: exact and numerical solutions (left), CPD map (center), and errors (right) for $I=41$ (shock location inside a cell) --- top/MOOD (the initial solution is the $\mathbb{P}_0$ solution with linear BC initial solution), bottom/AS (the initial solution is the MOOD solution).}
\begin{tabular}{ccc}
\includegraphics[width=0.31\textwidth]{exE/I41/out_NLSfsolveV3_7MOODNew5210_Var0-P0_article/res-I41-4MOOD-Rho_article} &
\includegraphics[width=0.31\textwidth]{exE/I41/out_NLSfsolveV3_7MOODNew5210_Var0-P0_article/res-I41-4MOOD-CPD_article} &
\includegraphics[width=0.31\textwidth]{exE/I41/out_NLSfsolveV3_7MOODNew5210_Var0-P0_article/res-I41-4MOOD-RhoError_article}\\
\includegraphics[width=0.31\textwidth]{exE/I41/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD_article/res-I41-11DS-Rho_article} &
\includegraphics[width=0.31\textwidth]{exE/I41/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD_article/res-I41-11DS-CPD_article} &
\includegraphics[width=0.31\textwidth]{exE/I41/out_NLSfsolveV3_8DSv1New5210_Var0-MOOD_article/res-I41-11DS-RhoError_article}
\end{tabular}
\end{table}


